Massively Parallel Computation in a Heterogeneous Regime

Massively-parallel graph algorithms have received extensive attention over the past decade, with research focusing on three memory regimes: the superlinear regime, the near-linear regime, and the sublinear regime. The sublinear regime is the most desirable in practice, but conditional hardness results point towards its limitations. In this work we study a \emph{heterogeneous} model, where the memory of the machines varies in size. We focus mostly on the heterogeneous setting created by adding a single near-linear machine to the sublinear MPC regime, and show that even a single large machine suffices to circumvent most of the conditional hardness results for the sublinear regime: for graphs with $n$ vertices and $m$ edges, we give (a) an MST algorithm that runs in $O(\log\log(m/n))$ rounds; (b) an algorithm that constructs an $O(k)$-spanner of size $O(n^{1+1/k})$ in $O(1)$ rounds; and (c) a maximal-matching algorithm that runs in $O(\sqrt{\log(m/n)}\log\log(m/n))$ rounds. We also observe that the best known near-linear MPC algorithms for several other graph problems which are conjectured to be hard in the sublinear regime (minimum cut, maximal independent set, and vertex coloring) can easily be transformed to work in the heterogeneous MPC model with a single near-linear machine, while retaining their original round complexity in the near-linear regime. If the large machine is allowed to have \emph{superlinear} memory, all of the problems above can be solved in $O(1)$ rounds.

==> algo_macros.tex <==
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\SetKwBlock{SmallMachines}{small machines do in parallel:}{end}
\SetKwBlock{LargeMachine}{large machine:}{end}
\SetKwBlock{LocallyCompute}{locally compute:}{end}
\SetKw{Disseminate}{disseminate}
\SetKw{Aggregate}{aggregate}
\SetKwFor{DoParallel}{for}{do in parallel}{end}
\SetKwFor{DoForEachParallel}{foreach}{do in parallel}{end}
\SetKwFor{ForPack}{for}{do}{end}


==> app_conn.tex <==

\section{Connectivity and $(1+\epsilon)$-approximation of MST in $O(1)$ Rounds}\label{app:conn}

In this section we show how by leveraging the existing techniques of linear sketches and $l_0$-sampling which are mostly used in the context of streaming algorithms (\cite{l0_sampling}, \cite{linearMeas}, \cite{linear_sket_stream_1}, \cite{linear_sket_stream_2}, \cite{linear_sket_stream_3}, \cite{linear_sket_stream_4}), as well as in the congested clique (\cite{connectivity_in_cc}), we get constant-round algorithms for connectivity and MST approximation in the \modelname{} model.
The implementation is very similar to the implementation in near-linear MPC, except that now the edges associated with a single vertex may be stored across more than a single machine;
using \emph{linear sketches}, this is trivial to overcome.

\begin{theorem} \label{conn_theorem}
There is an $O(1)$-round algorithm to identify the connected components of a graph with high probability in the \modelname{}.
\end{theorem}


\begin{proof}
We apply the connectivity algorithm from ~\cite{linearMeas} which is based on linear-sketches for $\ell_0$-sampling, as stated originally in \cite{l0_sampling},
but replacing the shared randomness assumed in~\cite{l0_sampling}
with $O(\log n)$-wise independence~\cite{linearMeas},
so that one machine can generate $O(\polylog n)$ random bits,
disseminate them to all the other machines,
and these are then used to generate all the sketches.
The sublinear machines compute a linear sketch $s(v)$ for each node $v \in V$. This sketch can be used to sample a random neighbor of $v$, and for a set of nodes $S = \{v_1,...,v_k\}$, the sketch $s = s(v_1) + ... + s(v_k)$ can be used to randomly sample an edge from $E[S,V \backslash S]$. The total number of bits required for all nodes sketches is $O(n\log^3(n))$, thus, all sketches can be stored in the near-linear-spaced machine which can then simulate the connectivity algorithm of \cite{linearMeas}. During the algorithm, nodes from the same connected component are merged using the sampled edges into contracted virtual nodes. The nodes in the final contracted graph represent the connected components of the input graph.  

In order to construct a sketch for some node $v$, it is required to know all neighbors of $v$. But, we cannot assume that the sublinear machine has a sufficient memory to hold all of $v$'s neighbors. Instead, we use the following property of the linear sketches:

\begin{property} \label{linearity_property}
Let $G_1,\dots,G_k \subseteq G$ such that $N(v) = N_{G_1}(v) \uplus \dots \uplus N_{G_k}(v)$, and let $s_1(v),\dots,s_k(v)$ be linear sketches in these graphs, then $s(v) = \sum_{i=1}^k s_i(v)$ is a linear sketch of $v$.
\end{property}

Each sublinear machine computes a partial-sketch for each $v \in V$ based on the neighbors of $v$ which it holds. Using Claim~\ref{aggregation_claim}, the final sketches are constructed by adding up all the partial sketches, which takes constant number of rounds.
\end{proof}

   

\begin{theorem}
For any constant $\epsilon > 0$, there is an $O(1)$-round algorithm to compute an $(1+\epsilon)$-approximation of the minimum spanning tree in the \modelname{}.
\end{theorem}

\begin{proof}
We follow the known reduction from \cite{linearMeas} to reduce the problem of estimating the weight of the minimum spanning tree to the problem of counting the number of connected components in the graph. This approach requires applying the connectivity algorithm in parallel over $O(\log(n))$ subgraphs. This takes constant number of rounds using the connectivity algorithm from theorem \ref{conn_theorem}.
\end{proof}

% Let $G$ be a graph with integral weights up to $W_{max} = \polylog(n)$. For each $0 \leq i \leq \log_{1+\epsilon}W_{max}$, let $G_i$ be a subgraph of $G$ induced by the edges of weight at most $(1+\epsilon)^i$.
% \begin{lemma}[\cite{linearMeas}]
% Let $T$ be a minimum spanning tree of G and set $r = \lceil \log_{1+\epsilon}W_{max} \rceil$. Then,
% \begin{equation*}
%     w(T) \leq n-(1+\epsilon)^r + \sum_{i=0}^r\lambda_i cc(G_i) \leq (1+\epsilon)w(T)
% \end{equation*}
% where $\lambda_i = (1+\epsilon)^{i+1} - (1-\epsilon)^i$ and $cc (G_i)$ is the number of connected components of graph $G_i$.
% \end{lemma} 
% So, it remains to compute $cc(G_i)$ for each $0 \leq i \leq \log_{1+\epsilon}W_{max}$ in $O(1)$ rounds. Apply the connectivity algorithm in parallel on each of the $\log_{(1+\epsilon)}W_{max}$ induced subgraphs $G_i$. By Theorem~\ref{conn_theorem}, this can be done in $O(1)$ rounds.
% \end{proof}


 


==> app_intro.tex <==
\section{The AMPC model}\label{sec:app_intro}
In the AMPC model, for an input of size $N$ there are $m$ machines, each with memory of size $S$, such that $m \cdot S = \Tilde{O}(N)$. Additionally, there is a collection of distributed data stores, denoted by $D_0, D_1, ...$, such that in the $i$'th round, each machine can read data from $D_{i-1}$ and
write to $D_i$. The number of bits a machine can read and write in one round is limited by $O(S)$. As opposed to the native MPC, it is not required for a machine to read all of the $O(S)$ bits at once in the beginning of the round. Instead, each machine can query bits based on previous queries that it has already made in the same round. This adaptive behavior was the reasoning for the model name. It was claimed by \cite{AMPC} that the AMPC model could actually be more practical than the general MPC in many cases. Specifically, they pointed out that the MPC model does not take into consideration the ability to perform RDMA operations, by which a data stored on a remote machine can be read with only a few microsecond latency without requiring a synchronized round of communication. The AMPC model tries to close this gap between theory and practice. Indeed, this model efficiently solves a few problems which were considered hard for the native MPC model. Among them are the minimum spanning tree problem, which can be solved in $O(\log\log_{\frac{m}{n}}(n))$ rounds, and maximal independent set, which can be solved in $O(1)$ rounds.

==> app_prelims.tex <==
\section{Missing Proofs from Section~\ref{sec:prelims}}\label{sec:app_prelims}
\subsection{Proof of Claims~\ref{aggregation_claim} and \ref{spreading_claim}.}
\begin{proof}

For concreteness we focus on the context of graph problems and assume that for all $1 \leq i \leq t$, the set $A_i$ is associated with some node $u \in V$. These assumptions hold in all the places we use Claim~\ref{aggregation_claim} through out the paper, but we note that the claim can be proved without them.

First, for each edge $(u,v) \in E$ we make two directed copies, $(u,v)$ and $(v,u)$. We sort all directed edges on the small machines
in lexicographic order.
Let $M_u$ be the first machine that
stores some outgoing edge of vertex $u$.
Each small machine $M$
sends to its successor 
the largest vertex $u$
such that some edge $(u,v)$ is stored
on $M$.
If $M$ holds some edge $(u,v)$ 
such that the predecessor of $M$
holds no outgoing edges of $u$, then 
$M$ informs the large machine that $M$
is the first machine that holds an outgoing
edge of $u$ (i.e., $M_u = M$).
Let $M'_u$ be the last machine that holds
some outgoing edge of $u$.
The large machine now knows the range of machines $[M_u, M'_u]$ that hold edges adjacent to $u$, for each $u \in V$.
Let $T_u$ be a tree 
with branching factor $n^{\gamma}$,
rooted at $M_u$,
whose nodes are the machines
in the range $[M_u, M_u']$,
such that for any two machines $M < M'$,
the depth of $M$ (its distance from the root)
is no greater than the depth of $M'$.
There are at most $n^{1-\gamma}$ machines that store outgoing
edges of $u$,
so the depth of $T_u$ is $O((1-\gamma)/\gamma)$.
We fix $T_u$ in advance as a function of $u$, $M_u$, $M'_u$. The large machine informs $M_u$ about the range $[M_u, M'_u]$. Then, the machine $M_u$ knows all its children in $T_u$ and what is the size of all its children's sub-trees, so it sends to each of its children the size of its sub-tree. By induction, each machine $M$ in the range $[M_u,M'_u]$ that receives the size of its sub-tree from its parent in $T_u$, knows all its children in $T_u$ and what is the size of all its children's sub-trees. So, in $O((1-\gamma)/\gamma)$ rounds all machines in the range $[M_u, M'_u]$ can know the IDs of 
their parent and their children in $T_u$. 
Note that $M$ can only be an inner node in one tree $T_u$:
if $M$ is not a leaf in $T_u$, then there is some machine $M'$ in $T_u$
whose depth is greater than $M$'s depth, meaning that $M < M'$
and so $M$
is not the last machine that stores outgoing edges of $u$;
there can be at most one node $u$ such that $M$ stores
some but not all edges of $u$.
Thus, each machine participates in at most one tree.

For the proof of Claim~\ref{aggregation_claim}, we have each machine $M$ in the leaf of the tree $T_u$ computes $f(B_u)$ such that $B_u \subseteq A_u$ is the set of elements that $M$ holds and send the computed value to its parent. Each inner-node machine computes $f(Y)$ such that $Y$ is the set of computed values received from all its children. The machine $M_u$, which is the root of $T_u$ will have the final result $f(A_u)$ in $O((1-\gamma)/\gamma)$ rounds.

To prove Claim~\ref{spreading_claim},
we disseminate a value $x_u$ to the machines in $T_u$ by having each machine in $T_u$ sending $x_u$ to all its children, starting from the root $M_u$. All the machines in $T_u$ that hold an element from $A_u$ will know the value $x_u$ in $O((1-\gamma)/\gamma)$ rounds.
    
\end{proof}

\subsection{Proof of Claim~\ref{consec_machines}}
\begin{proof}
    We sort all the edges using Claim~\ref{sorting_claim}.
    Next, using Claim~\ref{aggregation_claim},
    we compute the degree $\degout(v)$ of each node $v \in V$,
    using the
    domain $S = V \times \N$,
    the partition $\sett{ S_u = \sett{ u} \times \N }_{u \in V}$,
    the
    aggregation function $f(\sett{(u, x_1),\ldots,(u,x_t)}) = (u, \sum_{i = 1}^t x_i)$,
    and initial multiset $A = \sett{ (u,1) : (u,v) \in E, u < v }$.
    The small machines then report the node degrees
    to the large machines.
    Using this information,
    the large machine is able to identify the machine $M_{\mathrm{first}}(v)$ for each $v \in V$,
    and inform $M_{\mathrm{first}}$ itself.
\end{proof}

==> app_super_linear.tex <==
\section{Slightly Super-Linear Space}

\subsection{Minimum Spanning Tree}


\begin{proof}[proof of theorem~\ref{MST_with_super_lin}]
This is a generalization of the algorithm presented in Section~\ref{MST_section} that utilizes the extra memory of the large machine. Applying $t$ steps of exponential speed-up Bor{\r u}vka algorithm results in a contracted graph with $n' = \frac{n}{n^{2^tf(n)}}$ vertices (since in the $i$'th step, there is enough space in the large machine to hold up to $n^{2^if(n)}$ outgoing edges from each component). For the random-sampling step, we fix the sampling probability at $p=\frac{1}{n^{2^tf(n)+f(n)}}$, so that the number of light edges will be at most $O(n'/p) = O(n^{1+f(n)})$ which fits the memory of the large machine.
We get that for all $t \geq  \log(\frac{\log_n(m/n)}{f(n)})$, it holds that
\begin{equation*}
\begin{split}
    % m \cdot p = \frac{m}{ n^{2^tf(n)+f(n)}} \leq \frac{m}{n^{\log_n(m/n) + f(n)}} = \frac{m}{(m/n) + n^{f(n)}} = 
    & \frac{\log_n(m/n)}{f(n)} - 2 \leq \frac{\log_n(m/n)}{f(n)} \leq 2^t \\
    & \log_n(m/n) - 2f(n) \leq 2^tf(n) \\
    & \log_n(m/n) - f(n) \leq 2^tf(n) + f(n) \\
        & \frac{m}{n^{1+f(n)}} \leq n^{2^tf(n)+f(n)} \\
            &  \frac{m}{ n^{2^tf(n)+f(n)}} \leq n^{1+f(n)} \\
           & m \cdot p \leq n^{1+f(n)}
    \end{split}
\end{equation*}
and thus, after $O(\log(\frac{\log_n(m/n)}{f(n)}))$ iterations of Exponential speed-up Bor{\r u}vka, we can apply the final step of random-sampling (which takes constant number of rounds) to find the MST.

% and demand $m\cdot p \leq n^{1+f(n)}$. Thus, we get that:
% \begin{equation*}
% \begin{split}
%     &  \frac{m}{ n^{2^tf(n)+f(n)}} \leq n^{1+f(n)}  \\
%     & \frac{m}{n^{1+f(n)}} \leq n^{2^tf(n)+f(n)} \\
%     & \log_n(\frac{m}{n}) - f(n) \leq 2^tf(n)+f(n) \\
%      & \frac{\log_n(\frac{m}{n})}{f(n)} - 2 \leq 2^t \\
%      & \log(\frac{\log_n(\frac{m}{n})}{f(n)}) \leq t
% \end{split}
% \end{equation*}
% as claimed.


\end{proof}

\subsection{Maximal Matching}
\label{subsec:app_max_match}


\begin{proof}[proof of theorem~\ref{MM_with_super_lin}]
We follow the algorithm of \cite{filtering} for finding a maximal matching the MapReduce model. By \cite{filtering} Lemma~3.1, if we sample each edge of an input graph $G$ independently with some probability $p$ and find a maximal matching $M$ over the sampled subgraph $G_p$, the number of edges in $G$ whose both end-points are unmatched in $M$ (i.e., potentially can be added to the matching) is $O(n/p)$ with high probability. 

The algorithm is recursive. If the current graph has $O(n^{1+f(n)})$ edges, we reach the stop condition, and send all edges to the large machine to find a maximal matching. Otherwise, we sample each edge independently with probability $p = \frac{1}{n^{f(n)}}$ to create a random subgraph $G_p$. When the algorithm returns, a maximal matching $M$ of the graph $G_p$ is known to the large machine. The large machine notifies the small machines about the matched vertices in $M$ as described in Claim~\ref{spreading_claim}. Denote the set of edges that can potentially be added to the matching $M$ by $E_M$.
From the statement in the beginning of the proof, we have that $\vert E_M \vert = O(n^{1+f(n)})$, thus they can fit the memory of the large machine. Finally, the large machine computes the matching $M_2$ such that $M \subseteq M_2$ and returns $M_2$ from the recursive call. The algorithm takes at most $O(1/f(n))$ recursive iterations, at which point it reaches the stop condition.

\end{proof}
